How good are variational autoencoders at transfer learning?

Variational autoencoders (VAEs) are used for transfer learning across various research domains such as music generation or medical image analysis. However, there is no principled way to assess before transfer which components to retrain or whether transfer learning is likely to help on a target task. We propose to explore this question through the lens of representational similarity. Specifically, using Centred Kernel Alignment (CKA) to evaluate the similarity of VAEs trained on different datasets, we show that encoders' representations are generic but decoders' specific. Based on these insights, we discuss the implications for selecting which components of a VAE to retrain and propose a method to visually assess whether transfer learning is likely to help on classification tasks.

==> sections/app_latent.tex <==
\section{How well does CKA distinguish polarised regime from posterior collapse?}\label{sec:app-latents}

In~\Secref{subsec:res-hyperparameters}, we stated that CKA could be a useful tool to monitor posterior collapse.
Indeed, we have seen in~\Secref{subsec:bg-VAEs} that the polarised regime can be viewed as a ``healthy'' version of the posterior
collapse where the only latent variables that are not needed become passive, while posterior collapse will result in making
most of the latent variables passive, preventing the decoder from providing a good reconstruction.
In both cases, passive variables are close to $\N(0,1)$ in the sampled representation.~For this to be possible,
the mean representation of passive variables is always very close to 0, and the variance representation to 1,
so that the sampling process results in $\vz_i \approx \eps$ instead of $\vz_i = \mu_i + \sigma_i \eps$ where $\eps \sim \N(0,1)$.
While passive variables exhibit differences between the mean and sampled representations, the active variables are
very similar in mean and sampled representations. Indeed, in this case, the variance is very low, leading to $z_i \approx \mu_i$.

Keeping in mind that linear CKA is a generalisation of the correlation coefficient to matrices, if there is any linear
relationship between two representations, CKA will be high and the stronger this relationship is, the higher CKA will be.

Because mean and sampled representations have similar active variables but different passive variables, the presence of active
variables will result in higher CKA scores. Thus, mean and sampled representation will have higher CKA in polarised regime
(where they contain many active variables) than during posterior collapse (where there are none or very few active variables).
However, one can wonder whether CKA can lead to false positives when VAEs contain passive variables for
non-pathological reasons.~For example, due to the polarised regime, if one provides more latent variables than
needed by the VAEs, some of the variables will be collapsed to reduce the KL divergence.~As in posterior collapse, the decoder will
ignore these passive variables.~However, contrary to collapsed models, when passive variables are a result of the
polarised regime, the decoder will still have access to meaningful information and will be able to
correctly reconstruct the image, learning similar representations as a good model with fewer latent variables.
We can see in~\Figref{fig:latent-impact} that, in opposition to posterior collapse, the variance and sampled representations
retain much higher similarity scores with the representations learned by other layers.~Thus, one can differentiate between
the two scenarios using CKA. Given that the CKA scores for the variance and sampled representations vary similarly in fully-connected architectures,
CKA seems to consistently be a good predictor of posterior collapse across learning objectives and architectures while being
robust to false positives.
While one could be tempted to monitor posterior collapse using the changes of similarity scores in the decoder, we have seen in~\Appref{sec:app-fc}
that the fully-connected decoders could retain a relatively high similarity in the case of posterior collapse.
Thus, we recommend relying on the CKA scores of the mean, variance and sampled representations for a better robustness across architectures.

\begin{figure}[ht!]
    \centering
    \subcaptionbox{$\beta=1$\label{fig:latent-20}}{
        \includegraphics[width=0.5\textwidth]{heatmaps/dsprites/beta_vae_1_epoch_26_latent_10_beta_vae_1_epoch_26_latent_20}
    }%
    \subcaptionbox{$\beta=8$\label{fig:reg-10}}{
        \includegraphics[width=0.5\textwidth]{heatmaps/dsprites/beta_vae_1_epoch_26_beta_vae_8_epoch_26}
    }%
     \caption{(a) shows the CKA similarity scores between the activations of two $\beta$-VAEs trained on dSprites with $\beta=1$, the first with 10 latent variables, and the second with 20.
        (b) shows the CKA similarity scores between the activations of two $\beta$-VAEs with 10 latent variables trained on dSprites with $\beta=1$, and $\beta=8$.
        For (a) and (b), the activations are taken after complete training, and all the results are averaged over 5 seeds. We can see that we retain a higher similarity in the
        decoder representations in the case of polarised regime (bottom-right quadrant in (a)) than posterior collapse (see the darker bottom-right quadrant in (b)).
        The representational similarity of the mean, variance and sampled representations is also higher in the case of polarised regime than posterior collapse.}
    \label{fig:latent-impact}
\end{figure}


==> sections/app_vae.tex <==
\section{Additional details on mean, variance and sampled representations}\label{sec:app-vae}
This section presents a concise illustration of what mean, variance and sampled representations are.
As shown in~\Figref{fig:vae-archi}, the mean, variance and sampled representations are the last 3 layers of the encoder,
where the sampled representation, $\vz$, is the input of the decoder.~These representations, specific to VAEs, influence the models' behaviour that can be quite different from other deep learning models,
as shown by research on polarised regime and posterior collapse, for example.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.7\textwidth]{VAE_representations}
    \caption{The structure of a VAE}
    \label{fig:vae-archi}
\end{figure}

==> sections/checklist.tex <==
\section*{Checklist}
%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{This is discussed in~\Twosecrefs{subsec:bg-limitations}{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We discussed the environmental impact in~\Secref{sec:experiment} as well as the steps taken to mitigate them.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{The training details are given in~\Appref{sec:xp-setup} and the reason for their choice can be found in~\Secref{sec:experiment}.}
  \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{The shaded area of \Twofigref{fig:posterior-collapse}{fig:reg-encoder} show the variance over seeds. Not applicable for other figure types.}
  \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{This is done in~\Secref{sec:experiment}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{This is done in~\Secref{sec:experiment}.}
  \item Did you mention the license of the assets?
    \answerYes{We did mention dSprites licence in~\Secref{sec:experiment} but Cars3D and SmallNorb do not have any licence.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{The code URL is given in~\Secref{sec:intro}.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{The datasets used are open source.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{The datasets are synthetic.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}
